Unsupervised Hierarchical Grouping of Knowledge Graph Entities

Knowledge graphs have attracted lots of attention in academic and industrial environments. Despite their usefulness, popular knowledge graphs suffer from incompleteness of information, especially in their type assertions. This has encouraged research in the automatic discovery of entity types. In this context, multiple works were developed to utilize logical inference on ontologies and statistical machine learning methods to learn type assertion in knowledge graphs. However, these approaches suffer from limited performance on noisy data, limited scalability and the dependence on labeled training samples. In this work, we propose a new unsupervised approach that learns to categorize entities into a hierarchy of named groups. We show that our approach is able to effectively learn entity groups using a scalable procedure in noisy and sparse datasets. We experiment our approach on a set of popular knowledge graph benchmarking datasets, and we publish a collection of the outcome group hierarchies.

==> section/analysis.tex <==
\section{Optimal Loss in KGE Models}
\label{sec:analysis}

==> section/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

\clearpage

==> section/discussion.tex <==
\section{Results and Discussion}
\label{sec:discussion}

Table~\ref{table:fb15k_wn18_res} shows evaluation results for KGE models using different loss functions on the WN18 and NELL50k datasets. 
%
The results clearly show that changing cost function can improve the reported performance of the KGE models. Moreover, the functions we have proposed to optimise the model performance with respect to MRR behave exactly as assumed. 
%
%For all investigated KGE models, results show that model's version with original \ie default loss function does not provide best MRR compared to same model's versions with other loss functions.
%
For example, the TransE model originally uses the pairwise hinge loss, but the version with the tanh loss results in 1.7\% and 0.7\% MRR improvements on the WN18 and NELL50k datasets, respectively. DistMult also uses pairwise hinge loss by default, but its version with the PSL function achieve 1.2\% and 7.1\% better MRR scores. Finally, ComplEx originally uses pointwise logistic loss, but the version with ALS loss results in 0.9\% better MRR score on WN18, and its PSL version achieve 7\% better MRR on the NELL50k dataset.

In addition to confirming our main assumption, the results provide for an interesting observation. The versions of the TransE model with pairwise loss functions consistently achieve better results in terms of mean rank, MRR, and Hits@k when compared to the versions with pointwise losses. Conversely, DistMult and ComplEx models achieve best MRR and Hits@k scores with their versions that use pointwise losses. This behaviour is likely caused by the fact that the models use different scoring approaches. TransE scores triples using distances in the embedding space, but DistMult and ComplEx use a multiplicative approach. This observation may be used for designing optimal combinations of scoring and cost functions in future KGE models. However, for a truly comprehensive recommendation, more thorough analysis of other distance-based and multiplicative scoring functions is required.

In terms of the type of cost function, the results show that the models with our proposed pointwise square loss (PSL) function outperform their versions with other pointwise losses (the MRR score is better in 5 out of 6 experiment configurations of TransE, DistMult, and ComplEx models on both WN18 and NELL50k datasets). Regarding the pairwise loss, models using our proposed tanh and/or softsign loss functions provide better MRR score than other pairwise loss function in all experiment configurations.

An important technical observation is that the number of configurable parameters of a loss function has a significant impact on the time required for training the corresponding model. The training time grows exponentially with respect to the number of hyperparameters used in training. Pointwise ALS and both pointwise and pairwise logistic losses do not have configurable parameters, therefore they require minimal training time when compared to other losses with additional configurable parameters. Even the margin based loss functions that require only one parameter, $\lambda$, have significantly slower training time than ALS and logistic losses. In our experiments, models with configurable margin losses required 5 times more training time than model using losses with no configurable parameters. The tanh loss (with two configurable parameters, $\lambda$ and $\alpha$) required 25 times more training time than non parametric loss functions. 

The differences in evaluation accuracy of models using different loss functions can be sometimes relatively small. In real world large scale knowledge graph applications, the choice of training loss function for a KGE model will therefore always involve a compromise between both evaluation accuracy and training time efficiency.

In summary, our results clearly confirmed all our key assumptions. First of all, the choice of a loss function does have an impact on the performance of KGE models. Secondly, cost functions can be consciously selected in a way that can optimise particular evaluation metrics (we have focused on MRR in this paper since it is widely used for measuring the performance of the KGE models, but we plan to extend this for other metrics as well in future). This marks a big improvement over the state of the art approaches where the cost functions have been selected in a rather non-systematic way. Last but not least, we have brought up several interesting observations that can inform more rational and efficient design of future KGE models.



==> section/related.tex <==
\section{Background}
\label{sec:background}
 
\subsection{Loss functions in Learning to Rank}
\subsection{KGE Loss functions}
\subsection{Ranking Metrics}
\subsection{KGE Evaluation Protocol}


==> section/results.tex <==
\section{Results and Discussion}
\label{sec:results}
